Constraints First: A New MDD-based Model to Generate Sentences Under Constraints

This paper introduces a new approach to generating strongly constrained texts. We consider standardized sentence generation for the typical application of vision screening. To solve this problem, we formalize it as a discrete combinatorial optimization problem and utilize multivalued decision diagrams (MDD), a well-known data structure to deal with constraints. In our context, one key strength of MDD is to compute an exhaustive set of solutions without performing any search. Once the sentences are obtained, we apply a language model (GPT-2) to keep the best ones. We detail this for English and also for French where the agreement and conjugation rules are known to be more complex. Finally, with the help of GPT-2, we get hundreds of bona-fide candidate sentences. When compared with the few dozen sentences usually available in the well-known vision screening test (MNREAD), this brings a major breakthrough in the field of standardized sentence generation. Also, as it can be easily adapted for other languages, it has the potential to make the MNREAD test even more valuable and usable. More generally, this paper highlights MDD as a convincing alternative for constrained text generation, especially when the constraints are hard to satisfy, but also for many other prospects.

==> inc/algo.tex <==
\begin{algorithm}[tb]
\caption{MNREAD State}
\label{alg:intlog}
\fntitrealgo{createState}($state$, $label$) : State 

\Debut{}{

    $newState \gets $ \textsc{createState()} \\
    $newState.lenght \gets state.length + \#char(label)$ \\
    $newState.width \gets state.width + width(label)$ \\
    $newState.l1 \gets state.l1 $ \\
    $newState.l2 \gets state.l2 $ \\
    $newState.l3 \gets state.l3 $ \\
    $newState.lastcut \gets state.lastcut $  \\
    $newState.history \gets state.history[2:N]$ \\
    $newState.history[N] \gets label$ \\
    Return $newState$ \\
}


\fntitrealgo{isValid}($C$, $state$, $label$, $layer$) : Boolean

\Debut{}{
   Return $isValid\regleAffichage$ and $isValid\regleNombreCaracteres$ and $isValidNgram$ \\ 
}

\fntitrealgo{isValidBox}($C$, $state$, $label$, $layer$) : Boolean \\

\fntitrealgo{isValidLength}($C$, $state$, $label$, $layer$) : Boolean \\
\Debut{}{
If $layer = size-1$ \\
    Return $state.lenght + length(label)=59-size-1)$\\
        }
Return $state.lenght+ lenght(label)\leq59-size-1-layer$ \\        
\fntitrealgo{isValidLength}($C$, $state$, $label$, $layer$) : Boolean \\



\end{algorithm}

==> inc/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

\color{blue}
Generating text is perhaps the best known automatic natural language processing (NLP) task outside this research field.
Today, there are many language models that offer exceptional performance in the quality of the text produced.
Among the most recent, the transformers architecture and variants proposed for NLP achieve state-of-art results on benchmarks.
Classically, for a generation task, these models produce tokens (words) one by one following the probability distribution learned during the training phase.
Unfortunately, to date, this models does not allow to manage constraints on text production even though some experimental to modify this architecture in order to do so \ab{student abstract switch GPT}. By constraints we mean constraints defined in the sense of Constraint Programming (CP).
For the same reason that they are so effective on production :
there is no a priori reason to think that following a learned probability distribution on a dataset can solve an arbitrary constraint.
Especially, if the default dataset does not satisfy the constraint(s).
We address here the problem of generating text under constraints. More precisely, we propose to see the problem of generating text under constraints as a constraint satisfaction problem (CSP) with a CP approach. This precision is important because the word constraint is not understood in the same way in other fields.
\color{darkgreen}
For example, many recent works try to introduce "constraints", they usually rely on a beam search, while maximising the likelihood of the sequences, they try to satisfy the constraints (often lexical constraints, i.e., the occurrence of one or more words at a defined position in the generated sequence). We believe that this approach is appropriate as long as the solution space is weakly constrained.
But if we are interested in more constrained solution spaces this approach is just an ingenious heuristic workaround to a pure greedy search.

The interest of a CP approach is the paradigm reversal.
Defining constraints on a solution space is at the core of a CP resolution. But in return we lose a priori the undeniable statistical power of neural networks, but a posteriori we can still benefit from it (this idea will be developed in detail in the discussion section).
In this paper, we show that in the case of strongly constrained text generation, CP remains competitive with other methods and to do so we solve a real life problem.
\color{blue}
%In other words, the constraints considered are true for k words, but not for the entire sequence of n words. For example, a constraint of the type the word $W$ is present at position $i$ in the produced sequence $S_n$.
%This is perfectly sufficient when thinking about text generation in general. For example, "I want a sentence that starts with the", "I want the verb of the sentence in the source language to be translated into a verb of a more formal language level in the target language". On the other hand, if we are interested in a property on the sequence such as "I want the sum of the characters of the words in the sequence to be equal to $s$. This view of constraints becomes inefficient for a problem like this, conversely it is straightforward in CP. And it is precisely in this kind of consideration that the CP paradigm excels. 

To illustrate our approach, we are interested in the production of standardised sentences (which satisfy a sharp protocol, i.e., a set of strict rules ) used in an extremely well-known reading test used in the field of vision research: the MNREAD reading test.


%Moreover, we consider our constraints to be strong for two reasons: (i) they may be linguistic, but also size, or display. That is to say, we go beyond the more general rules on text. (ii) we are interested in constraints on the text which make it almost impossible to find in what has already been written.

\color{black}

Since reading performance has become one of the most widely used clinical measures to judge the effectiveness of treatments, surgical procedures, or rehabilitation techniques. This reading performance is measured by the time taken to read standardized texts, i.e., texts designed to be equivalent in terms of length, display, and linguistics. This need for equivalent texts is the key to avoiding bias in the texts themselves. In addition, each text should only be presented once to the subjects or patients to avoid recall bias and ensure accurate measurement.

Among the various tests, the MNREAD test \cite{mansfield-ahn-etal:93} is probably one of the most widely used standardized reading tests in the world for measuring reading performance in clinical and research settings in people with normal or low vision.
For instance, it is used to evaluate how reading performance depends on font size~\cite{calabrese-owsley-etal:16}. An MNREAD test comprises standardized sentences printed in 19 sizes in 0.1 logMAR increments (an angular unit that quantifies visual acuity). 
It is available in 19 languages, with various tests depending on the language (e.g., five English, two French). Since repeated measurements are needed in many MNREAD applications, the scientific and medical communities need a large number of test sets, mainly to avoid recall bias. Unfortunately, this is impossible today because the number of MNREAD sentences is largely insufficient. 

Increasing the number of MNREAD sentences is a complex problem because
of the multiple rules the sentences must follow. Writing these sentences
or ﬁnding them in corpora is not the solution because they are
particular. So particular that almost no existing instances satisfy all the rules: out of a sample of more than three million
sentences from children's literature, only four satisfy the criteria of
the MNREAD reading test. A first idea to solve this rule-dominated problem would be to use deep learning methods (e.g., Transformers), which are in full expansion \ab{citation} However, they might be challenging to implement in our case for the following two reasons~: (i) they require large learning bases, but we only have a small number of original MNREAD sentences, and (ii) to our knowledge, the introduction of rules (constraints) in deep networks poses limitations, but this is a fast-evolving topic at the moment;
\color{blue}
(iii) several attempts have been made to guide a beam search with a transformers model like GPT-2. However, three limitations push us to think differently to tackle our problem (a) the constraint usually considered in a beam are way weaker than ours. (b) beam search is a heuristic; we want an exact method (c) there is no reason to think that the sentences that satisfy the constraints are the sentences considered likely by the transformers. Thus, our method first relies on solving the constraints and then selecting the best sentences. \color{black} \ab{note ajouter citations}



Another idea is to design more ad-hoc approaches dedicated to reading tests~\cite{crossland-legge-etal:07,perrin-paille-etal:15,mansfield-atilgan-etal:19}. In particular, in~\cite{mansfield-atilgan-etal:19}, the authors, who are also the creators of the MNREAD test, propose an approach based on sentence templates ({\itshape templates}) and capable of generating millions of sentences using a random walk. 
However, this semiautomatic method has several major drawbacks: (i) it relies on sentence templates that have
to be created manually (i.e., sequences of placeholders, each containing
a list of possible words that ﬁt into the sentence at a deﬁned
position); (ii) it requires a manual verification of the sentences generated by the system; (iii) it cannot be easily extended 
to other languages, as for French, where one has to take into
account agreements and conjugations or other languages that use
declension (e.g., German, Baltic language, Slavic); (iv) since the
sentences generated are based on templates, the number of different
words are restrained. Thus, it may lead to a memory bias for readers.

We propose to model the standardized text generation problem as a constrained satisfaction problem to overcome these limitations. The goal is to have a more automatic approach (without the need to define a sentence model {\itshape a priori}), which produces only sentences respecting the rules (without having to check them {\itshape a posteriori}), and finally which can be generalized (i.e., with other rules or in other languages). For this purpose, we propose an original approach based on multi-valued decision diagrams (MDDs). 
MDDs have already been successfully used in many other problems, such as the generation of music~\cite{roy-perez-etal:16} or poems~\cite{perez-regin:17b}. Other uses of MDDs for optimization problems can be found in the reference work of Bergman et al.~\cite{bergman-cire-etal:16}, or in the more recent thesis of Perez~\cite{perez:17}. 
MDDs are a generalization of binary decision diagrams (BDDs)~\cite{akers:78}. 
They are data structures for computing and storing solutions (tuples) of a problem using an directed acyclic graph (DAG).
Using MDDs in our context offers four main advantages~: 
(i) MDDs allow representing a large number of solutions in a compressive structure, which will be crucial given the size of the data we will have to manipulate,
(ii) MDDs allow the problem to be decomposed by defining as many MDDs as there are rules that the text must respect;
(iii) it is possible to perform operations between MDDs efficiently and without decompressing them, thus allowing for the combination of different rules;
(iv) in addition, MDD is a straightforward extension and an efﬁcient way of representing a corpus (i.e., the succession of words of a text) in a compressed manner.

In this paper, we consider reduced ordered MDD. Then MDDs are structured in layers where each layer represents an ordered variable $X_i$.
There are two particular nodes in the MDD: the root (\nroot) and the true terminal node (\ntt). Each path between the node \nroot and \ntt forms a label tuple which corresponds to a valid assignment of the variables associated with each layer. The label $l_{a_{k}}$ of the arc $a_k$ belonging to any path between the layer $i-1$ and $i$ is the assignment of the variable $X_i$ such that $X_i$ = $l_{{a}_k}$. 
A path $p$ = ($a_1$, $a_2$, $a_3$, $\ldots$, $a_r$) exists in the MDD if and only if the variable assignment $X_i$=$l_{a_{i}}$ is valid for all $i$. 
Thus calculating an MDD containing $r$ layers is equivalent to calculating the valid $r$-uplets of the function $f : \{0...d\}^r \mapsto \{true,false\}$.
x An example of an MDD of type sum is given in Fig. \ref{fig:exemple-MDD-type-somme}.
\begin{figure}[htbp]
  \begin{center}
    \includegraphics[width=0.25\textwidth]{ima/MDD_sum_cropped.png}
  \end{center}
\caption{\label{fig:exemple-MDD-type-somme}
Example of MDD representing the set of %solutions 
$x_1 + x_2 + x_3 \in [5,9]$.
For each variable $x_i$, the domain $D(.)$ is %well defined:
$D(x_1)$ = $\{1,3,7\}$, $D(x_2)$ = $\{0,2,4\}$, $D(x_3)$ = $\{2,3,4\}$.
For example, $(7,0,2)$ belongs to the set of solutions belonging to the MDD. }
\end{figure}


MDDs could describe all combinations between words to
construct sentences. However, to have a better chance of obtaining
syntactically correct sentences, the idea is to consider only
recombining existing sentence fragments. More precisely, given a corpus
made up of a set of sentences written by authors (whose syntax and
meaning are therefore correct), the usual idea is to decompose them into
n-grams (a subsequence of \emph{n} words built from a given sentence).
From the sentence: ``He lives in a nice little red house''. We can ﬁnd
several 3-grams (e.g., a nice little, nice little red, little red house...). On top of that, we can link two n-grams if the $n-1$ last words of the first \ngram are the $n-1$ first words of the second \ngram. Then sentences are obtained by following links between n-grams. An MDD will be responsible for containing the sentences (combinations of n-grams). In addition, there will be other MDDs (one for each rule that the text must respect) responsible for resolving the constraints on the text. To obtain our MNREAD sentences, we make the intersection of the different MDDs. Finally, we select the sentences having meaning.

The plan of this article is as follows.
Section Our Approach shows how to model the constrained text generation problem with MDDs. To illustrate this, we focus on the generation of MNREAD sentences. We start with a reminder of the MNREAD rules. Then we explain how to construct the associated MDDs, and, finally, how to intersect them.
The experimental results are presented in section Results, in which we show the potential of our method. We continue with a Discussion section where we explain some perspectives that enhance this work, and we end with a Conclusion.


==> inc/introduction2.tex <==
\section{Introduction}
\label{sec:introduction}

We consider the problem of generating text under constraints.
%The ouput must satisfies a set of defined rules. This is a constrained text generation task. 
Currently, the methods for solving this problem are mainly based on two foundations:
(a) Language Models (LM) that have been proven on a number of tasks\footnote{https://gluebenchmark.com/} \cite{glue:2018} in natural language processing (NLP) (b) a side component to perform a filtering or a search on the text generated by (a). More preciselly, theses use Beam Search (BS) for mainly lexical and semantic constraint (\cite{beamsearch1:2021} \cite{beamsearch2:2018} \cite{hokamp-liu:2017}). Recently a new method introduce an A* search instead of BS \cite{lu-etal-2022-neurologic} and sometimes constraints (like Oulipo\footnote{https://en.wikipedia.org/wiki/Oulipo} rules) can be handle by token (words) filtering (\cite{roush-etal-2022-language}.
%(c) A RETIRER POUR LE MOMENt: some works also go in the direction of adding the constraints directly in the architecture of (a).
These search-based heuristics involve generating the text word by word while maximizing the likelihood of the sequence computed by (a) and checking the constraints with (b).
This approach is appropriate as long as the solution space is weakly constrained i.e., it is easy to find a sequence satisfying the constraints. This is usually the case for lexical or semantic constraint. Conversely, in the case of a strongly constrained solution space such as precise and clear requirements in the output (e.g., display constraint, length constraint) it is way harder to find a sequence satisfying the constraints, and we must proceed differently. In this case, it is better to first check the constraints and then select the best solutions with (a), because there is no reason that the sequences that (a) consider likely would satisfy the constraint.


%\begin{figure}[htbp]
%    \centering
%    \includesvg[width=0.45\textwidth]{ima/schema.svg}
%    \caption{This drawing summarizes our point of view about the constrained text generation task. We are in the blue zone if the problem is weakly constrained and implicitly has lots of potential instances that satisfy the constraints. If the number of constraints increases and reduces the potential solutions spaces, then we are in the green zone. Hence, this paper will develop ideas considering this situation.}
%        \caption{The constrained text generation task. The blue area represents the problems for which the constraints are easy to satisfy, while the green area represents those for which finding a solution satisfying the constraints is difficult. 
%This paper will develop ideas considering this situation.}
%    \label{fig:schemaconstraint}
%\end{figure}


%In other words, if the goal is guided by coherence and quality of the text, (a) is suited. If some side constraints are added (b) is sufficient.

We can see constrained text generation problem as a discrete combinatorial optimization problem, where variables are words, domain of variables is vocabulary of the text and contraints are the set of rules that the text has to satisfy. This formulation generalizes a previous similar idea developped in a paper where the authors address the problem of generating very long palindromes \cite{papadopoulos:2015} (creativity is at his sake).

In this paper, we propose a Constraint Programming (CP) model for solving a constrained text generation problem and show its effectiveness through the MNREAD sentences generation problem. The MNREAD sentences generation problem consists of producing standardized sentences satisfying a sharp protocol ( i.e., a set of strict rules ). 
These sentences are used to build the MNREAD reading test which is a well-known test in the field of vision research for measuring reading speed. Increasing the number of MNREAD sentences is a complex problem because of the several hard constraints the sentences must follow. Writing these sentences
or ﬁnding them in corpora is not the solution because they are
particular. So particular that almost no existing instances satisfy all the rules: out of a sample of more than three million 
sentences from children's literature (600 books), only four satisfy the criteria of the MNREAD reading test. %Therefore, another approach must be investigated.


Even though we want to satisfy the constraints first, applying a pure {\itshape{generate and test}} over random words would find sequences satisfying the constraints but those sequences would not have a meaning. In other words, these sequences are not "well-formed" sentences. Since we cannot totally ignore the language structure, we rely on combining existing sequences of words (n-grams). From the sentence: ``He lives in a nice little red house'', we can ﬁnd
several 3-grams (e.g., a nice little, nice little red, little red house...).  On top of that, we can link two n-grams if the $n-1$ last words of the first \ngram are the $n-1$ first words of the second \ngram. Then sentences are obtained by following links between n-grams. %Papadopolous et al. start from ngram to build the greatest palindromes \cite{papadopoulos-roy-etal:14}

Our approach is based on multi-valued decision diagrams (MDDs) to produce sentences. An MDD is a well suited data structure to store and retrieve successions of \ngrams. Also, using MDD provide a way to compute an exhaustive set of solutions without performing a search. Therefore, our approach is an exact method.
% XXX from which the best ones are selected with Transformers.
In addition, we use a Language Model (LM) to select the best sentences.
An LM is a probabilistic model used to predict the sequence of words in a text or speech using natural language training data. Here we use transformers-based LM (i.e., LM implementing Transformers architecture based on attention block \cite{vasmani-et-al:2017}). More specifically, we use GPT-2 \cite{radford:2019}, which has been trained over a tremendous amount of text and is designed to generate sequences. GPT-2 is also suited to assess sentence quality to a certain degree by assigning a score to sequences. We use this score to sort sentences and select the best ones. It drastically simplifies human verification and, in the best case, avoids it.

The paper is organized as follows: in section \ref{sec:prelim}, we give some preliminaries. We start with a reminder of the MNREAD rules and MDDs.
Then in the section \ref{sec:methode}, we show how to model the constrained text generation problem with MDDs.
We also explain how to use an LM to select the best sentences.
The experimental results are presented in the section \ref{sec:resultats}, in which we show the potential of our method.
At last, in the section \ref{sec:discussion}, we share additional thoughts on this work and give some perspectives on future investigations.
Finally, we conclude.



%More precisely, we consider constrained text generation as a constrained satisfaction problem (CSP). In other words, we model the words as a set of variables, any rules on texts as a set of constraints\footnote{In CP terminology, constraints are a logical properties that cannot be violated}, and the allowed vocabulary as domains associated to the variables.


%It is available in 19 languages, with various tests depending on the language (e.g., five English, two French). Since repeated measurements are needed in many MNREAD applications, the scientific and medical communities need a large number of test sets, mainly to avoid recall bias. Unfortunately, this is impossible today because the number of MNREAD sentences is largely insufficient. 

%Increasing the number of MNREAD sentences is a complex problem because of the multiple rules the sentences must follow. 

%Writing these sentences or ﬁnding them in corpora is not the solution because they are particular. So particular that almost no existing instances satisfy all the rules: out of a sample of more than three million sentences from children's literature, only four satisfy the criteria of the MNREAD reading test.

%A first idea to solve this constraints-dominated problem would be to use pure ML (e.g., Transformers), which are in full expansion \ab{citation} However, they might be challenging to implement in our case for the following two reasons~: (i) We only have a small number of original MNREAD sentences, and (ii) to our knowledge, the introduction of constraints in ML especially neural networks poses limitations, but this is a fast-evolving topic at the moment;
%On the other hand, as we mention as starting point of the introduction several attempts have been made to guide a beam search with a transformers model like GPT-2. However, three limitations push us to think differently to tackle our problem (a) the constraint usually considered in a beam are way weaker than ours. (b) beam search is a heuristic; we want an exact method (c) there is no reason to think that the sentences considered likely by the transformers are the sentences that satisfy our constraints.

%Another idea is to design more ad-hoc approaches dedicated to reading tests~\cite{crossland-legge-etal:07,perrin-paille-etal:15,mansfield-atilgan-etal:19}. In particular, in~\cite{mansfield-atilgan-etal:19}, the authors, who are also the creators of the MNREAD test, propose an approach based on sentence templates ({\itshape templates}) and capable of generating millions of sentences using a random walk. 
%However, this semiautomatic method has several major drawbacks: (i) it relies on sentence templates that have to be created manually (i.e., sequences of placeholders, each containing a list of possible words that ﬁt into the sentence at a deﬁned position); (ii) it requires a manual verification of the sentences generated by the system; (iii) it cannot be easily extended to other languages, as for French, where one has to take into account agreements and conjugations or other languages that use declension (e.g., German, Baltic language, Slavic); (iv) since thesentences generated are based on templates, the number of different words are restrained. Thus, it may lead to a memory bias for readers.

%Our goal is then to have a more automatic approach (without the need to define a sentence model {\itshape a priori}), which produces only sentences respecting the rules (without having to check them {\itshape a posteriori}), and finally which can be generalized (i.e., with other rules or in other languages). For this purpose, we propose an original approach CP-based on multi-valued decision diagrams (MDDs). 
%MDDs have already been successfully used in many other problems, such as the generation of music~\cite{roy-perez-etal:16} or poems~\cite{perez-regin:17b}. Other uses of MDDs for optimization problems can be found in the reference work of Bergman et al.~\cite{bergman-cire-etal:16}, or in the more recent thesis of Perez~\cite{perez:17}. 

==> sty/myinformation.tex <==
\newcommand{\articletitle}{Constrained text generation to measure reading performance: A new approach based on multivalued decision diagrams}

==> sty/sourceGraphviz.tex <==

digraph {
    rankdir="LR"
    subgraph MDDmot {
	graph [nodesep="0.3", ranksep="0.3",fontsize=12]
	node [shape=circle, fontsize=12]
	edge [arrowsize=0.6]

	0 [label="root"]


	3 [label=""]
	4 [label="3"]
	5 [label=""]
	6 [label="", color="black"]
	7 [label=""]
	8 [label="", color="black"]
	121 [label="8"]
	122 [label="8"]
	30 [label=""]
	20 [label=""]
	

	14 [label=""]
	151 [label="",color="white"]
	152 [label="",color="white"]
	1512 [label="11",color="black"]
	153 [label="",color="white"]
	154 [label="",color="white"]
	155 [label="",color="white"]
	156 [label="",color="white"]
	
    252 [label="16",color="black"]
    2512 [label="",color="white"]
	
	156 [label="",color="white"]
	
    
    
	0->5 [label="He"]
    0->20 [label= "cat"]
	0->6 [label="white",color="black", fontcolor="black"]
	0->4 [label="The, 3"]
	0->3 [label="A"]
	
	
	20->30 [label="loves"]
	3->14 [label=" red"]
	4->121 [label=" black, 5"]
	4->122 [label=" white, 5"]
	5->7 [label=" loves"]
	6->8 [label=" cat",color="black", fontcolor="black"]
	
	7->155 [label="you"]
	8->156 [label="loves", color="black", fontcolor="black"]

    30->151 [label="milk"]
	121->152 [label="cat, 3"]
	122->1512 [label="cat, 3"]
	14->153 [label="apple"]
	14->154 [label="car"]
	
	1512->252 [label="loves, 5",color="darkgreen",fontcolor="darkgreen"]
	
	
	
    }
}




digraph {
    subgraph MDDmot {
	graph [nodesep="0.3", ranksep="0.3",fontsize=12]
	node [shape=circle, fontsize=12]
	edge [arrowsize=0.6]

	0 [label="root"]


	3 [label=""]
	4 [label=""]
	5 [label=""]
	6 [label="", color="black"]
	7 [label=""]
	8 [label="", color="black"]
	9 [label=""]
	10 [label=""]
	11 [label=""]
	12 [label=""]

	
	15 [label="tt"]
    
    0->3 [label="cat"]
    0->4 [label="white", color="blue"]
    0->5 [label="He"]
    0->6 [label="The", color="red" ]
    0->7 [label="A"]
    
    3->8 [label=" loves"]
    4->9 [label=" cat", color="blue"]
    5->10 [label="loves", ]
    6->11 [label="white", color="red"]
    6->11 [label=" black"]
    7->12 [label=" red"]
    
    8->15 [label="milk"]
    9->15 [label="loves", color="darkgreen", fontcolor="darkgreen"]
    10->15 [label="you"]
    11->15 [label="cat", color="red"]
    12->15 [label="car"]
    12->15 [label="apple"]
    


    }
}


digraph {
    subgraph MDDmot {
	graph [nodesep="0.3", ranksep="0.3",fontsize=12]
	node [shape=circle, fontsize=12]
	edge [arrowsize=0.6]

	0 [label="root"]


	3 [label=""]
	4 [label=""]
	5 [label=""]
	6 [label="", color="black"]
	7 [label=""]
	8 [label="", color="black"]
	9 [label=""]
	10 [label=""]
	11 [label=""]
	12 [label=""]

	
	15 [label="tt"]
    
    0->3 [label="cat"]
    0->4 [label="white", color="blue",fontcolor="blue"]
    0->5 [label="He"]
    0->6 [label="The", color="red",fontcolor="red" ]
    0->7 [label="A"]
    
    3->8 [label=" loves"]
    4->9 [label=" cat", color="blue",fontcolor="blue"]
    5->10 [label="loves", ]
    6->11 [label="white", color="red",fontcolor="red"]
    6->11 [label=" black"]
    7->12 [label=" red"]
    
    8->15 [label="milk"]
    9->15 [label="loves", color="darkgreen", fontcolor="darkgreen"]
    10->15 [label="you"]
    11->15 [label="cat", color="red",fontcolor="red"]
    12->15 [label="car"]
    12->15 [label="apple"]
    


    }
}


digraph {
    
    subgraph MDDmot {
	graph [nodesep="0.3", ranksep="0.3",fontsize=12]
	node [shape=circle, fontsize=12]
	edge [arrowsize=0.6]

	0 [label="root"]


	3 [label=""]
	4 [label="3"]
	5 [label=""]
	
	7 [label=""]
	
	121 [label="8"]
	122 [label="8"]

	

	14 [label=""]
	151 [label="",color="white"]
	152 [label="",color="white"]
	1512 [label="11",color="black"]
	153 [label="",color="white"]
	154 [label="",color="white"]
	155 [label="",color="white"]
	156 [label="",color="white"]
	
    252 [label="16",color="black"]
    2512 [label="",color="white"]
	
	156 [label="",color="white"]
	
    
    
	0->5 [label="He"]
    
	
	0->4 [label="The, 3"]
	0->3 [label="A"]
	
	
	
	3->14 [label=" red"]
	4->121 [label=" black, 5"]
	4->122 [label=" white, 5"]
	5->7 [label=" loves"]
	
	
	7->155 [label="you"]
	

    
	121->152 [label="cat, 3"]
	122->1512 [label="cat, 3"]
	14->153 [label="apple"]
	14->154 [label="car"]
	
	1512->252 [label="loves, 5",color="darkgreen",fontcolor="darkgreen"]
	
	
	
    }
}







\begin{table}[t]
\centering
\small
\begin{tabular}{|l|l|}
\hline
English Generated Sentences & PPL \\
\hline
%You should be able to get in and out of the back of the bus &9.3 \\
%And he had no idea what to do with the fact that she was in &9.7 \\
It was as if she was trying to figure out what had happened &9.8 \\
And the fact that he was standing in the middle of the room &10.2 \\
She closed her eyes and shook her head as if she was afraid &10.6 \\
%And do you think it would be nice to be able to keep an eye &10.7 \\
Aside from the fact that we were in the middle of the night &10.8 \\
It was as though he had no idea what to do or where to look &10.9 \\
.... & ... \\
The old fellow who owns the place is a bit of a temperature &93 \\
The family in front of the double doors and into the branch &100 \\
The difference here was now she had to deal with it tonight &108 \\
Staying low and as much as it is to the edge of a high drop &111 \\
So much for seeing the end of the table to steady her hands &136 \\
She caught sight of the back of beyond just to write a book &281 \\

\hline
\end{tabular}
\caption{\label{tab:sentences_scoring_en} example of generated english sentences sorted by PPL score using gpt-2 \tablefootnote{https://huggingface.co/gpt2}
}
%\end{table}
%
\ \\ 
%\begin{table}[htbp]
\centering
\small
\begin{tabular}{|l|l|}
\hline
French Generated Sentences & PPL \\
\hline
Assise à la table de la salle à manger il y a un bon moment & 6.23 \\
Elle se pencha vers elle et lui donna un grand coup de pied & 6.62 \\
Et il y a des choses dont on ne peut pas dire la même chose & 6.82 \\
Nous avons à peine le temps de faire un tour dans la maison & 6.83 \\
Ses parents ne sont pas au courant de la maladie de sa mère & 6.94 \\
.... & ... \\
Il frappa à nouveau dans ses yeux et de voir la grue bouger & 230 \\
La poupée finit par tomber sur le sol et préparai mon bâton & 241 \\
Une hache reposait près de lui et de ne pas jouer aux héros & 241 \\
Quand le bout de la salle et frappa dans ses mains en coupe & 242 \\
Une hache reposait près de lui et de ne pas sortir ensemble & 291 \\
\hline
\end{tabular}
\caption{\label{tab:sentences_scoring_fr} example of french generated sentences sorted by PPL score using asi/gpt-fr-cased-base\tablefootnote{https://huggingface.co/asi/gpt-fr-cased-base}
}
\ \\ 
 \centering
     \begin{tabular}{|l|l|}
     \hline
Sentences & PPL \\
\hline
Le policier passa la main dans sa poche et se mit à marcher &23 \\
Le policier passa la main dans sa poche et se mit à compter &26 \\
Le policier passa la main dans la poche arrière de mon jean &38 \\
Le policier passa la main dans la poche de son jean déchiré &42 \\
Le policier passa la main dans la poche de sa nouvelle robe &76 \\
        \hline
        
     \end{tabular}
    \caption{\label{tab:exemple-de-phrases-avec-meme-amorce} Examples of sentences generated in 5-grams with the same sentence start.}
\end{table}

